Model Predictive Control Strategies for Electric Endurance Race Cars Accounting for Competitors Interactions

This paper presents model predictive control strategies for battery electric endurance race cars accounting for interactions with the competitors. In particular, we devise an optimization framework capturing the impact of the actions of the ego vehicle when interacting with competitors in a probabilistic fashion, jointly accounting for the optimal pit stop decision making, the charge times and the driving style in the course of the race. We showcase our method for a simulated 1h endurance race at the Zandvoort circuit, using real-life data of internal combustion engine race cars from a previous event. Our results show that optimizing both the race strategy as well as the decision making during the race is very important, resulting in a significant 21s advantage over an always overtake approach, whilst revealing the competitiveness of e-race cars w.r.t. conventional ones.

==> Report/Titlepage.tex <==
\begin{titlepage}
	\centering
	\vspace*{0.5 cm}
	\includegraphics[width = 120mm]{Figures/Logo.eps}\\[0.5 cm]		% University Logo
	\textsc{\LARGE Eindhoven University of Technology}\\[2.0 cm]% University Name
	\textsc{\Large Master thesis}\\[0.5 cm]							% Course Code
%	\textsc{\large Graduation project}\\[0.5 cm]			% Course Name
	% 	{\bfseries Department of Mechanical Engineering\\}
	\rule{\linewidth}{0.2 mm} \\[0.4 cm]
	{\huge\bfseries Maximum-distance Race Strategies for a Fully Electric Endurance Race Car\\}
	%{\huge\bfseries \hl{Report Title Continuation} \\ }
	\rule{\linewidth}{0.2 mm} \\[1.5 cm]
	
	
	\begin{minipage}{0.4\textwidth}
		% \vspace{0.5cm}
		%\includegraphics[width=0.7\linewidth]{Figures/cover.png}\\[10pt]
		\centering
		% {\Large\bfseries Authors }\\[5pt]
		%\begin{table}[H]
		% \centering
		%   \label{authors}
		
		%  \begin{minipage}{0.4\textwidth}
			\begin{flushright} \normalsize
				
				Master \\
				Department \\
				Research group \\[1cm]
				\emph{Authors}\\
				\textsc{van Kampen} J.H.E.\\[1cm] % Name
			\end{flushright}
		\end{minipage}
		\hspace{1cm}
		\begin{minipage}{0.4\textwidth}
			\begin{flushleft} \normalsize
				
				Automotive Technology \\
				Mechanical Engineering \\
				Control Systems Technology\\[1cm]
				\emph{Student numbers} \\
				0952110\\ %student 
			\end{flushleft}
		\end{minipage}\\[2cm]
		\emph{Supervisor}\\
		dr. ir. M.R.U. Salazar Villalon\\[2cm]
		
		Eindhoven, \today
		
		%\begin{flushright}
		%    \vfill
		%	\hl{Supervised by}\\
		%	\hl{Name, \textsc{TU Eindhoven}}
		%\end{flushright}	
		\newpage
		\includegraphics[width=\linewidth]{Report/Code_of_conduct.pdf}
		\newpage
	\end{titlepage}
